Privacy-Preserving Model and Preprocessing Verification for Machine Learning

This paper presents a framework for privacy-preserving verification of machine learning models, focusing on models trained on sensitive data. Integrating Local Differential Privacy (LDP) with model explanations from LIME and SHAP, our framework enables robust verification without compromising individual privacy. It addresses two key tasks: binary classification, to verify if a target model was trained correctly by applying the appropriate preprocessing steps, and multi-class classification, to identify specific preprocessing errors. Evaluations on three real-world datasets-Diabetes, Adult, and Student Record-demonstrate that while the ML-based approach is particularly effective in binary tasks, the threshold-based method performs comparably in multi-class tasks. Results indicate that although verification accuracy varies across datasets and noise levels, the framework provides effective detection of preprocessing errors, strong privacy guarantees, and practical applicability for safeguarding sensitive data.

==> sections/motivation.tex <==

\section{Motivation}\label{sec:motivation}

When evaluating the performance of a machine learning model, one commonly used metric is overall accuracy. While accuracy provides a broad measure of how well the model performs on a given dataset, it can be insufficient for a comprehensive assessment. Accuracy alone may fail to capture important nuances in the model’s behavior, particularly in complex tasks or imbalanced datasets.

To gain a more detailed understanding of model performance, one often turns to additional metrics. In the context of classification tasks, a confusion matrix is a valuable tool that breaks down the model's predictions into true positives, false positives, true negatives, and false negatives. From this matrix, one can derive numerous performance metrics beyond accuracy, such as precision, recall, F1-score, and others. These metrics provide a more constructive view of the model’s strengths and weaknesses, offering insights into how well the model distinguishes between different classes.

However, even with these detailed metrics, there is a risk of bias. In a classification task, the confusion matrix and the metrics derived from it are heavily influenced by the distribution of the testing set. If the testing set is biased or not representative of the diversity or characteristics of real-world data or a specific user's dataset, the metrics may appear favorable yet fail to reveal underlying flaws in the model.

To address this limitation, we propose leveraging prediction explanations to evaluate model behavior. Unlike traditional performance metrics, prediction explanations are not affected by the distribution of the testing set. They provide insight into the model's decision-making process, highlighting the features or patterns that influence its predictions. This approach allows us to verify the model’s behavior in a more transparent and unbiased manner (see Table~\ref{tab:motivation_table}).

Our proposed method involves using prediction explanations from a verifier's model to train a machine learning classifier, which is then used to assess whether the target model behaves similarly. Additionally, we calculate the cosine distance between the explanations generated by the verifier’s model and the target model. A significant distance between these models can indicate discrepancies or errors in the target model's behavior. This single distance metric is more intuitive for users from various backgrounds, as it simplifies the verification process and reduces the need for deep knowledge of multiple performance metrics.

Furthermore, this method enhances data privacy. The verifier does not need access to the true labels of the shared data, which protects the privacy of the target model's dataset. Additionally, the testing set does not need to be large or perfectly balanced, as the focus is on comparing model behavior rather than relying on a representative testing set. This efficient approach not only simplifies the verification process but also reduces the effort and expertise required to ensure the integrity of machine learning models.



\begin{table*}[ht]
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}{|l|p{6.5cm}|p{6.5cm}|}
\hline
\textbf{Criteria} & \textbf{Explanations \& Cosine Distance} & \textbf{Traditional Performance Metrics} \\ \hline
\textbf{Interpretability} & Intuitive; one metric & Requires understanding multiple metrics \\ \hline
\textbf{Dependence on Testing Set} & Less dependent on test set & Highly dependent on test set \\ \hline
\textbf{Bias Detection} & Identifies subtle biases & May miss biases if test set is unbalanced \\ \hline
\textbf{Privacy} & No need for true labels or balanced test set & Requires true labels and balanced test set \\ \hline
\textbf{Implementation Complexity} & Simple; focuses on one metric & Complex; involves multiple metrics \\ \hline
\textbf{Generalizability} & Reflects diverse model behavior & Limited to test set distribution \\ \hline
\end{tabular}
\caption{Comparison of Explanations \& Cosine Distance vs. Performance Metrics}
\label{tab:motivation_table}
\end{table*}









